SurvAttack: Black-Box Attack On Survival Models through Ontology-Informed EHR Perturbation

Survival analysis (SA) models have been widely studied in mining electronic health records (EHRs), particularly in forecasting the risk of critical conditions for prioritizing high-risk patients. However, their vulnerability to adversarial attacks is much less explored in the literature. Developing black-box perturbation algorithms and evaluating their impact on state-of-the-art survival models brings two benefits to medical applications. First, it can effectively evaluate the robustness of models in pre-deployment testing. Also, exploring how subtle perturbations would result in significantly different outcomes can provide counterfactual insights into the clinical interpretation of model prediction. In this work, we introduce SurvAttack, a novel black-box adversarial attack framework leveraging subtle clinically compatible, and semantically consistent perturbations on longitudinal EHRs to degrade survival models' predictive performance. We specifically develop a greedy algorithm to manipulate medical codes with various adversarial actions throughout a patient's medical history. Then, these adversarial actions are prioritized using a composite scoring strategy based on multi-aspect perturbation quality, including saliency, perturbation stealthiness, and clinical meaningfulness. The proposed adversarial EHR perturbation algorithm is then used in an efficient SA-specific strategy to attack a survival model when estimating the temporal ranking of survival urgency for patients. To demonstrate the significance of our work, we conduct extensive experiments, including baseline comparisons, explainability analysis, and case studies. The experimental results affirm our research's effectiveness in illustrating the vulnerabilities of patient survival models, model interpretation, and ultimately contributing to healthcare quality.

==> tex/Survival.tex <==


\section{Preliminary of Survival Analysis}
%The main outcome of survival analysis studies is the Survival Function S(t), which represents the probability of surviving beyond time t

%By optimizing the time-independent partial likelihood, the CPH model focuses on the order of the events but not on the actual event times.

%The predicted survival function of a subject who developed the event is compared to: (1) that of subjects who developed the event before his=her survival time, and (2) that of subjects who developed the event, or were censored, after ,his=her survival time. Subjects who were censored are involved in comparisons with subjects who developed the event before their observed times.

%in its handling of censored data and
%"failure time",
\iffalse
Survival analysis (SA) \cite{cox1972regression} is a statistical method used to analyze and predict the time until an event of interest, often referred to as "survival time", or "event time". It is distinct as it focuses on the time until an event occurs, rather than whether it occurs, and also in its handling of censored data (unlabeled data) as a semi-supervised task. Censored data refers to cases where the occurrence of the event has not been observed for some subjects during the study period, whereas for observed data (labeled data) the event of interest is observed within the study period. 
\fi
%Early survival analysis started from the Cox proportional hazards (CPH) \cite{10.2307/2985181} model and its extensions  \cite{lin2002modeling, fine1999proportional, JMLR:v20:18-424} due to CPH's simplicity and interpretibility. Later, there comes other advanced methods such as Random Survival Forests \cite{ishwaran2008random}, Bayesian models\cite{fernandez2016gaussian}, and most importantly deep learning-based methods such as DeepHit \cite{lee2018deephit, lee2019dynamic}, Survtrace \cite{wang2022survtrace}, OTCSurv \cite{nayebi2023contrastive}, and many more. 

%Early in survival analysis, the Cox proportional hazards (CPH) \cite{10.2307/2985181} model was prominent, assuming a proportional relationship between covariates and hazard. The simplicity and interoperability of CPH, led to various Cox-based survival model extensions \cite{lin2002modeling, fine1999proportional, JMLR:v20:18-424}. Also, other approaches have been used for time modeling in survival analysis such as Random Survival Forests \cite{ishwaran2008random}, Bayesian models\cite{fernandez2016gaussian}, and most importantly deep learning-based methods such as DeepHit \cite{lee2018deephit, lee2019dynamic}, Survtrace \cite{wang2022survtrace}, OTCSurv \cite{nayebi2023contrastive}, and many more. 

%Survival analysis is widely employed to model the time until an event of interest occurs. 

%\begin{equation}
%   S(t|V) = P_{V}(\tau>t)
%\end{equation}

Survival models aim to estimate the survival function $S(t|V) = P_{V}(\tau>t)$ that represents the probability that an individual will survive beyond a specific time point $t$ given the subject's covariate $V$. In survival analysis, the mean lifetime denoted as $\mu$, representing the average time until an event occurs, is computed by integrating the survival function over time, 
%\begin{equation}
    $\hat{T} = \int_{0}^{\infty} S(t|V) \, dt.$
%\end{equation}
We consider $\hat{T}$ as the predicted survival time duration and also the output of the victim survival models in the following sections.


\iffalse
Another important concept in SA is the hazard function, denoted as $\lambda(t)$, characterizing the instantaneous rate at which the event occurs at time t, given that it hasn't occurred before. Mathematically, it's defined as:
\vspace{-3ex}
\begin{equation}
    %f(t|x) = P_{x}(T=t)
    \lambda(t) = \lim_{{\Delta t \to 0}} \left[ \frac{P(t \leq T < t + \Delta t \,|\, T \geq t)}{\Delta t} \right]
\end{equation}

Survival function $S(t)$ can also be derived from Hazard function $\lambda(t)$ as follows:
\begin{equation}
    S(t) = \exp\left(-\int_{0}^{t} h(u) \, du\right)
\end{equation}
\fi



The objective of attacks on survival models is to undermine the survival model's ranking capability and compromise survival time prediction. 
The following two survival analysis metrics are monitored to assess attack effectiveness in achieving its goals.

%\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
First, the Concordance Index (c-index), which is used to assess concordance or agreement between the predicted survival times ranking and that of the actual survival times. A higher c-index indicates better concordance, meaning that the model's predicted rankings align more closely with the actual survival outcomes. %It quantifies the model's ability to correctly rank or discriminate between subjects with different survival times. 
%The C-index measures the proportion of pairs of subjects in the dataset for which the predicted survival times are correctly ranked. 
Consider a pair of subjects $(i, j)$ with the actual survival times of $T_{i}$ and $T_{j}$, predicted survival times of  $\hat{T}_{i}$ and $\hat{T}_{j}$, and censoring labels of $k_{i}$ and $k_{j}$ (censored $k=0$, observed $k=1$). To compute the c-index, we consider three types of patient pairs: 
\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]
\item Patients in the pair are both observed subjects ($k_{i} = k_{j} = 1$). We say $(i, j)$ is a concordant pair if $T_{j} > T_{i}$ and $\hat{T}_{j} > \hat{T}_{i}$ (correct ranking prediction), a discordant pair if $T_{j} > T_{i}$ and $\hat{T}_{j} < \hat{T}_{i}$ (incorrect ranking prediction), and a tied pair if $\hat{T}_{j} = \hat{T}_{i}$.

\item Patients in the pair are both censored subjects ($k_{i} = k_{j} = 0$). They are excluded from the computation because it's impossible to determine who experienced the event first (unrankable).

\item Patient $i$ is a censored subject and patient $j$ is an observed subject ($k_{i} = 0, k_{j} = 1$). If $T_{j} > T_{i}$, the pair is excluded because, again, it's unclear who experienced the event first. If $T_{j} < T_{i}$, $(i, j)$ is a concordant pair if $\hat{T}_{j} < \hat{T}_{i}$, a discordant pair if $\hat{T}_{j} > \hat{T}_{i}$, and a tied pair if $\hat{T}_{j} = \hat{T}_{i}$. 
\end{enumerate}

Given the defined pairs, Harrell’s C-index is defined as:
\begin{equation}
    C=\frac{\sum_{i, j} \left[\mathrm{I}\left(\hat{T}_i<\hat{T}_j\right) + 0.5\cdot\mathrm{I}\left(\hat{T}_i=\hat{T}_j\right) \right] \cdot \mathrm{I}\left(T_{i}<T_{j}\right) \cdot {k}_j}{\sum_{i, j} \mathrm{I}\left(T_{i}<T_{j}\right) \cdot {k}_i}
\end{equation}
which is the number of concordant pairs plus half the number of tied pairs, divided by the number of permissible (rankable) pairs. The operator $I(condition)$ is an indicator function that returns $1$ for true conditions and $0$ otherwise.

%In survival analysis, assessing the model's ability to predict survival times (regression) is crucial, but it can only be evaluated for observed data. 
The second metric, Mean Absolute Error (MAE), measures the accuracy of time predictions for observed data:
\begin{equation}
    %MAE = \|T_{i} - \hat{T}_{i}\|
    \text{MAE} = \frac{1}{N_\text{ob}} \sum_{i=1}^{N_\text{ob}}\|T_{i} - \hat{T}_{i}\|
\end{equation}
where $N_\text{ob}$ is the number of observed subjects.
%\end{itemize}


